MART: Learning Hierarchical Music Audio Representations with Part-Whole Transformer

Recent research in self-supervised contrastive learning of music representations has demonstrated remarkable results across diverse downstream tasks. However, a prevailing trend in existing methods involves representing equally-sized music clips in either waveform or spectrogram formats, often overlooking the intrinsic part-whole hierarchies within music. In our quest to comprehend the bottom-up structure of music, we introduce MART, a hierarchical music representation learning approach that facilitates feature interactions among cropped music clips while considering their part-whole hierarchies. Specifically, we propose a hierarchical part-whole transformer to capture the structural relationships between music clips in a part-whole hierarchy. Furthermore, a hierarchical contrastive learning objective is crafted to align part-whole music representations at adjacent levels, progressively establishing a multi-hierarchy representation space. The effectiveness of our music representation learning from part-whole hierarchies has been empirically validated across multiple downstream tasks, including music classification and cover song identification.

==> apendix.tex <==



We selected a specific music example named "mrdc-timecode-01-lust-175-204.mp3" from MTAT. This music audio file has several labels to portray its characteristics, including "electronic", "beat", "vocal", "male vocal", "female vocal", and "pop". Its waveform is shown in Figure \ref{fig:case1}. "Electronic" and "pop" labels are whole-level traits, which are tagged by the red box. "Female", "vocal", "male", and "beat" are part-level traits reflected in different clips, which are tagged by the green, purple, and orange boxes, respectively. Therefore, we devised Music-PAW to represent part-whole hierarchies of music, which can help the model perceive the hierarchies of music characteristics more accurately. Our model can better understand music, thus improving the performance of downstream tasks.

\begin{figure}[t]
    \centering
        \includegraphics[width=\linewidth]{figures/case1.pdf}
    \caption{The waveform of a music audio selected from MTAT dataset. We use several boxes with different colors to tag its labels of the different parts.}
    \label{fig:case1}
\end{figure}


In Section \ref{subsec:model_analysis}, Figure \ref{fig:visual} shows that the Baseline model fails to distinguish music of different hierarchies, which are also irregularly distributed. In contrast, the representations of different hierarchies from the same music in Music-PAW are more distinguishable and exhibit noticeable intra-hierarchy clusters. Specifically, in the multi-label music classification task, the part-level representations of the Baseline model mix up with the whole-level representations. This shortcoming means that the Baseline model cannot clearly perceive the part-level traits and the whole-level traits of music when tagging music. In other words, part-level and whole-level representations can only reflect one of the part-level or whole-level traits. However, the part-level representations of Music-PAW are more distinguishable and are not far away from the whole-level representations simultaneously. Therefore, when Music-PAW utilizes the part-level representations to tag part-level traits for music, it can also perceive the whole-traits of music. Thus, Music-PAW can recognize the all traits of music more accurately.






==> related_work.tex <==
% \subsection{Self-supervised Learning.}
\vpara{Self-supervised Learning.} Self-supervised Learning (SSL) targets learning representations from the vast unlabeled data through hand-crafted pretext tasks. For instance, context prediction \cite{Doersch2015, Devlin2019}, image jigsaw puzzle \cite{Noroozi2016}, predicting the image's rotation \cite{Gidaris2018}, and reconstruction \cite{Goodfellow2020, Baldi2012, Donahue2019, Brock2019}. Although these methods have demonstrated their validity, the learned representations lack generalization. The recent contrastive learning methods \cite{Caron2020, Hadsell2006, Henaff2019, Tian2020, He2020, Chen2020, Grill2020, Zbontar2021, Misra2019, Kalantidis2020, Chuang2020, Hu2021} have made much progress in self-supervised learning. For example, MoCo \cite{He2020} views contrastive learning as a dictionary look-up to build a dynamic queue, including samples of the current and previous mini-batch. Another method SimCLR \cite{Chen2020}, is a simple framework for contrastive learning without a memory bank. BYOL \cite{Grill2020} proposed a new paradigm for contrastive learning, which only used positive samples while casting away negative samples.


%In the past, most of contrastive learning methods are based on the instance discrimination task \cite{Wu2018} in which positive samples are specified as different views of the same objective, while negative samples are constituted by sampling views from different objectives. Since \cite{Hadsell2006} whose approaches contrast positive pairs against negative pairs to learn representation, contrastive learning has attracted a great deal of attention from both academia and the industrial community. 

%Contrastive Predictive Coding \cite{Henaff2019} is an unsupervised objective that learns predictable representation. CMC \cite{Tian2020} is view-agnostic and can scale to any number of views by maximizing mutual information between different views of the same observation for learning representation. MoCo \cite{He2020} views the contrastive learning as a dictionary look-up to build a dynamic queue including samples of the current mini-batch and the previous mini-batch and a moving-averaged encoder. Another method SimCLR \cite{Chen2020}, is a simple framework for contrastive learning without a memory bank. Recently, BYOL \cite{Grill2020} proposed a new architecture for contrastive learning, which consists of online and target networks. They train the networks only with the various augmented views of an identical image without negative pairs. To avoid collapsed solution and minimize the redundancy, \cite{Zbontar2021} contrast samples from features dimension.


%\subsection{Music and Audio Representation Learning.}
\vpara{Music and Audio Representation Learning.} Benefiting from contrastive self-supervised learning, which has been applied to learn visual representations \cite{He2020, Chen2020, Grill2020, You2020,Qiu2020, Jansen2018} and has achieved outstanding performance, some works \cite{Wang2021,Al-Tahan2020,Saeed2021,Niizumi2021,Spijkervet2021} with regard to using contrastive learning methods to learn music and audio representations have emerged recently. CLMR \cite{Spijkervet2021}, CLAR \cite{Al-Tahan2020}, COLA \cite{Saeed2021} and Multi-Format\cite{Wang2021} expand their work in SimCLR \cite{Chen2020} contrastive framework to learn audio representations. Another contrastive paradigm, BYOL \cite{Grill2020}, which casts away the negative pairs during the pre-training stage, has also been employed to obtain auditory representations by BYOL-A \cite{Niizumi2021}. Apart from these works, wave2vec \cite{Schneider2019} and wave2wec 2.0 \cite{Baevski2020} have explored how to obtain the representation of speech. 

% CLMR \cite{Spijkervet2021} select the raw waveform of audio segments as its inputs. CLAR \cite{Al-Tahan2020} and \cite{Wang2021} maximizes the similarity between the raw signals and the spectrogram from the same audio data. COLA \cite{Saeed2021} minimizes the distance between two augmented views from the same entire audio data in contrastive space. 

% In addition to these audio representation learning methods, musicBERT \cite{Zeng2021} understands music audio through music notes sequence. After that, a namesake model musicBERT \cite{Zhu2021} has been proposed to learn music structure via extracting beat feature from music audio. 


%\subsection{Part-whole Hierarchies.} 
% \vpara{Part-whole Hierarchies.} Several studies have attempted to capture part-whole hierarchies for visual representation. \cite{Tu2006} is the first attempt to parse an image into a part-whole hierarchy. Recently, Hinton \cite{Hinton2021} has proposed an imaginary system GLOM, which answers how a neural network can parse an image into a part-whole hierarchy. After that, ViP \cite{Sun} is proposed to divide visual representations into part-level and whole-level. Likewise, \cite{Garau2022} devises a framework capable of providing a representation of part-whole hierarchies from visual cues. Hip \cite{Carreira2022} introduces a sequence of splitting-processing-merging blocks to process information at different hierarchical levels. 
%In addition, in the audio domain, Jukebox \cite{Dhariwal2020} utilizes hierarchical structure to generate music.
